Tackling the Saturation of Oxygen: The Use of Phosphorus and Sulphur as Proxies Within the Neutral Interstellar Medium of Star-Forming Galaxies

The abundance of oxygen in galaxies is widely used in furthering our understanding of galaxy formation and evolution. Unfortunately, direct measurements of O/H in the neutral gas are extremely difficult to obtain, as the only OI line available within the Hubble Space Telescope (HST) UV wavelength range (1150-3200 A) is often saturated. As such, proxies for oxygen are needed to indirectly derive O/H via the assumption that solar ratios based on local Milky Way sight lines hold in different environments. In this paper we assess the validity of using two such proxies, PII and SII, within more typical star-forming environments. Using HST-Cosmic Origins Spectrograph (COS) far-UV (FUV) spectra of a sample of nearby star-forming galaxies (SFGs) and the oxygen abundances in their ionized gas, we demonstrate that both P and S are mildly depleted with respect to O and follow a trend, log(PII/SII)= -1.73+/-0.18, in excellent agreement with the solar ratio of log(P/S)_sol=-1.71+/-0.04 over the large range of metallicities (0.03-3.2 Z_sol) and H I column densities (log[N(H I)/cm^-2] =18.44-21.28) spanned by the sample. From literature data we show evidence that both elements individually trace oxygen according to their respective solar ratios across a wide range of environments. Our findings demonstrate that the solar ratios of log(P/O)_sol=-3.28+/-0.06 and log(S/O)_sol=-1.57+/-0.06 can both be used to derive reliable O/H abundances in the neutral gas of local and high-redshift SFGs. The difference between O/H in the ionized- and neutral-gas phases is studied with respect to metallicity and H I content. The observed trends are consistent with galactic outflows and/or star formation inefficiency affecting the most metal-poor galaxies, with the possibility of primordial gas accretion at all metallicities.

==> Ndens_HOPS.tex <==
\begin{table}
\begin{center}
\begin{scriptsize}
\caption{Logarithmic Column Densities of \hi, \oi, \pii, \& \sii\, within the Sample} \label{tab:Ndens}
%\title{Properties of Sample}
\begin{tabular}{lcccc}
\tableline\tableline
Galaxy	&	log[$N$(\hi)]			&	log[$N$(\oi)]			&	log[$N$(\pii)]			&	log[$N$(\sii)]			\\
 %& /cm$^{-2}$  & /cm$^{-2}$  & /cm$^{-2}$  & /cm$^{-2}$ \\
\tableline
I~Zw~18	&	21.28	$\pm$	0.03	& $>$	14.80	&	\ldots			&	14.72	$\pm$	0.05	\\
SBS~0335$-$052	&	21.70	$\pm$	0.05	& $>$	14.77	&	12.96	$\pm$	0.15	&	14.96	$\pm$	0.03	\\
SBS~1415+437	&	21.09	$\pm$	0.03	& $>$	14.87	&	13.41	$\pm$	0.08	&	14.94	$\pm$	0.03	\\
NGC~4214	&	21.12	$\pm$	0.03	& $>$	15.25	&	13.74	$\pm$	0.04	&	15.55	$\pm$	0.03	\\
NGC~5253-Pos.1	&	21.20	$\pm$	0.01	& $>$	15.44	&	13.73	$\pm$	0.08	&	15.43	$\pm$	0.02	\\
NGC~5253-Pos.2	&	20.65	$\pm$	0.05	& $>$	15.31	&	13.60	$\pm$	0.12	&	15.33	$\pm$	0.04	\\
NGC~4670	&	21.07	$\pm$	0.08	& $>$	15.26	&	13.80	$\pm$	0.05	& $>$	15.58			\\
NGC~4449	&	21.14	$\pm$	0.03	& $>$	15.54	&	14.09	$\pm$	0.09	&	15.60	$\pm$	0.09	\\
NGC~3690$_{v1}$	&	20.62	$\pm$	0.02	& $>$	15.48	&	\ldots			&	15.39	$\pm$	0.05	\\
NGC~3690$_{v2}$	&	19.81	$\pm$	0.08	& $>$	14.84	&	\ldots			&	\ldots			\\
M83-Pos.1	&	19.59	$\pm$	0.32	&	\ldots	&	13.84	$\pm$	0.26	&	15.39	$\pm$	0.25	\\
M83-Pos.2	& $<$	18.44			&	\ldots	& $<$	13.73			& $<$	15.39			\\\tableline
\end{tabular}
\\[1.5mm]
Notes:  All column densities refer to ICF-corrected values. 
%(see text for details).  ICFs were found to be negligible for log[N(\hi)/cm$^{-2}$]$\,\gtrsim\,20$.
\end{scriptsize}
\end{center}
\end{table}
